Diversity-Multiplexing Tradeoff in Selective-Fading Multiple-Access MIMO Channels

We establish the optimal diversity-multiplexing (DM) tradeoff of coherent selective-fading multiple-access multiple-input multiple-output (MIMO) channels and provide corresponding code design criteria. As a byproduct, on the conceptual level, we find an interesting relation between the DM tradeoff framework and the notion of dominant error event regions which was first introduced in the AWGN case by Gallager, IEEE Trans. IT, 1985. This relation allows to accurately characterize the error mechanisms in MIMO fading multiple-access channels. In particular, we find that, for a given rate tuple, the maximum achievable diversity order is determined by the error event that dominates the total error probability exponentially in SNR. Finally, we show that the distributed space-time code construction proposed recently by Badr and Belfiore, Int. Zurich Seminar on Commun., 2008, satisfies the code design criteria derived in this paper.

==> defs.tex <==
\newcommand{\eref}[1]{(\ref{#1})}                  

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\beqa}{\vspace{0mm} \begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray} \vspace{0mm}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

\newcommand{\bpr}{\noindent\emph{Proof.} }
\newcommand{\epr}{\hspace{\stretch{1}} $\square$}

\newcommand{\lefto}{\mathopen{}\left}
\newcommand{\sizebrackets}[1]{\lefto[ #1 \right]}
\newcommand{\sizeparentheses}[1]{\lefto( #1 \right)}
\newcommand{\sizecurly}[1]{\lefto\{ #1 \right\}}



\newcommand{\mt}{\mathrm{M_T}} 					
\newcommand{\mr}{\mathrm{M_R}} 						
\newcommand{\minant}{\mathrm{m}} 			
\newcommand{\maxant}{\mathrm{M}} 				
\newcommand{\channelH}{{\matc{H}}} 
\newcommand{\channelHw}{\matc{H}_{\mspace{-2.0mu}w}} 
\newcommand{\channelHwbar}{\overline{\matc{H}}_{\mspace{-2.0mu}w}}

\newcommand{\setR}{\mathbb{R}}                                
\newcommand{\setS}{\mathcal{S}}        
\newcommand{\set}[1]{\setS_{#1}}                           

\newcommand{\cn}[2]{\mathcal{CN}\negthinspace\left(#1,#2\right)}            
\newcommand{\mean}[1]{\mathbb{E}\negthinspace\left\{#1\right\}}             
\newcommand{\meansub}[2]{\mathbb{E}_{#1}\left\{#2\right\}}     

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}  
\newcommand{\matc}[1]{\bv{\mathcal{#1}}}                             
\newcommand{\bv}[1]{\mbox{\boldmath{$#1$}}}                     
\newcommand{\msf}[1]{\mathsf{#1}}													
\newcommand{\mbb}[1]{\mathbb{#1}}	
												
\newcommand{\rank}[1]{\mathrm{rank}\negthinspace\left(#1\right)}
\newcommand{\vecop}[1]{\mathrm{vec} \lefto(#1\right)}            
\newcommand{\expf}[1]{\exp{\negmedspace\sizeparentheses{#1}}}                    
\newcommand{\trace}[1]{\mathrm{Tr}\left(#1\right)}              
\newcommand{\diag}[1]{\mathrm{diag}\negthinspace\left\{#1\right\}}             

\newcommand{\mutinf}{\mathrm{I}}                                 
\newcommand{\jensen}{\mathrm{J}}                                    
\newcommand{\logdet}[1]{\log\det\left(#1\right)}  
\newcommand{\snr}{\msf{SNR}}                                 
\newcommand{\dotleq}{\mathrel{\dot{\leq}}} 
\newcommand{\dotl}{\mathrel{\dot{<}}} 
\newcommand{\dotg}{\mathrel{\dot{>}}} 
\newcommand{\dotgeq}{\mathrel{\dot{\geq}}} 

\newcommand{\pieigexp}[2]{\Lambda_{#1}^{#2}}
\newcommand{\pieig}{\Lambda_\minant^{{\rho \mathrm{M}_{\scriptscriptstyle{\mathrm{T}}}}}} 
\newcommand{\mutinfexp}[2]{\log\det\negthinspace\left(\mat{I}_{#1}+ #2 \right)}      

\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)} 
\newcommand{\outage}{\mathcal{O}}  
\newcommand{\joutage}{\mathcal{J}}
\newcommand{\pout}{P_\mathcal{\scriptscriptstyle O}}                            
\newcommand{\pjout}{P_\mathcal{\scriptscriptstyle J}}
\newcommand{\dout}{d_\mathcal{\scriptscriptstyle O}}                               
\newcommand{\djout}{d_\mathcal{\scriptscriptstyle J}}

\newcommand{\codebook}{\mathcal{C}}                                          
